Reallocation Problems with Minimum Completion Time

Reallocation scheduling is one of the most fundamental problems in various areas such as supply chain management, logistics, and transportation science. In this paper, we introduce the reallocation problem that models the scheduling in which products are with fixed cost, non-fungible, and reallocated in parallel, and comprehensively study the complexity of the problem under various settings of the transition time, product size, and capacities. We show that the problem can be solved in polynomial time for a fundamental setting where the product size and transition time are both uniform. We also show that the feasibility of the problem is NP-complete even for little more general settings, which implies that no polynomial-time algorithm constructs a feasible schedule of the problem unless P$=$NP. We then consider the relaxation of the problem, which we call the capacity augmentation, and derive a reallocation schedule feasible with the augmentation such that the completion time is at most the optimal of the original problem. When the warehouse capacity is sufficiently large, we design constant-factor approximation algorithms under all the settings. We also show the relationship between the reallocation problem and the bin packing problem when the warehouse and carry-in capacities are sufficiently large.

==> intro.tex <==
{\large\bf Problem setting}: Suppose that there are several warehouses that store many products (or items). 
Some of the  products are already stored at the designated warehouses, and the others are stored at tentative warehouses. Such temporally stored  products should be reallocated to designated warehouses. Namely, each  product $p$ at the tentative warehouse $s(p)$ is required to be reallocated to the designated warehouse $t(p)$. To reallocate  product $p$, it takes a certain length of time $\tau(p)$, called transit time of $p$.  
Each  product $p$ also has size $size(p)$,  and each warehouse has three kinds of capacities, that is, (1) the capacity of warehouse itself,  (2) carry-in size capacity, and (3) carry-out size capacity. Capacity (1) restricts the total size of  products stored in a warehouse at each moment. Capacities (2) and (3) restrict the total size of  products that are simultaneously carried in and out, respectively. In this setting, we consider the problem of finding a reallocation schedule with minimum completion time. 
 
As an illustrative  example of our problem, let us consider the following scenario. 
There are 6  products $p_1, p_2, p_3, p_4, p_5$ and $p_6$ of sizes $1, 3, 5, 6, 3$ and $4$, respectively. 
Two warehouses $W_1$ and $W_2$ have the warehouse capacities $20$ and $10$, carry-in capacities $6$ and $5$, and carry-out capacities $5$ and $5$, respectively. 
The transit time satisfies  $\tau(p_i)=1$ for every $i$ except $i=6$, and $\tau(p_6)=2$.  
Initially,  products $p_1, p_2, p_3$ and $p_4$ are stored in $W_1$, 
which satisfies the warehouse capacity constraint, since  their total size $15$ is smaller than the warehouse capacity $20$ of $W_1$.
Products $p_5$ and $p_6$ are initially stored in $W_2$, which also satisfies the warehouse capacity constraint. Suppose that $p_1, p_2$ and $p_3$ are designated to be stored in $W_2$, whereas $p_4$, $p_5$ and $p_6$ are designated to be stored in $W_1$. 
Note that all  products can be stored in the designated warehouses, since the designated allocation satisfies the warehouse capacity constraint. 
%The total size $13$ of $p_4, p_5, p_6$ is less than 20 the capacity of $W_1$, 
%and  the total size $9$ of $p_1,p_2,p_3$ is also less than the capacity $10$ of $W_2$; the total capacities of $W_1$ and $W_2$ are satisfied in the designated warehouses. 
We also note that $p_1,p_2$ and $p_3$ cannot be moved simultaneously, since the carry-out capacity constraint is violated. Figure \ref{fig:example} depicts the initial and target configurations of this example.  
\begin{figure}[hbtp]
%  \begin{minipage}[b]{0.40\linewidth}
%    \centering
%    \includegraphics[keepaspectratio, width=60mm]{fig/warehouse1.png}
%    \caption{Initial configuration} \label{fig:example1}
%  \end{minipage}
%  \hspace*{1cm}
%  \begin{minipage}[b]{0.40\linewidth}
%    \centering
%     \includegraphics[keepaspectratio, width=60mm]{fig/warehouse2.png}
%    \caption{Target configuration} \label{fig:example2}
%  \end{minipage}
    \centering
     \includegraphics[keepaspectratio, width=130mm]{fig/warehouse0.png}
     \caption{Example: initial (left) and target (right) configurations.} \label{fig:example}
\end{figure}

In this example, 
%a possible schedule is to carry out $p_1$ and $p_2$ from $W_1$, and $p_6$ from $W_2$ at time $0$, 
we need to move $p_1$, $p_2$ and $p_3$ to $W_2$, which should be done separately due to carry-out constraint $5$. Thus we consider to move $p_1$ and $p_2$ at time $0$ and then move $p_3$ at time $1$, for example. In such a case, we also need to move either $p_5$ or $p_6$ to $W_1$ at time $0$, otherwise it violates capacity $10$ of warehouse $W_2$ at time $1$. Thus a possible schedule is to carry out $p_1$ and $p_2$ from $W_1$, and $p_5$ from $W_2$ at time $0$, and then carry out $p_3$ from $W_1$ and $p_6$ from $W_2$ at time $1$. The completion time is $3$ in this case, because $\tau(p_6)=2$ and thus $p_6$ reaches $W_1$ at time $3$. One may consider that it is better to carry out $p_6$ instead of $p_5$ at time $0$ and then carry out $p_5$ at time $1$, but it violates carry-in constraint $6$ of $W_1$ at time $2$. By this observation, we can see that the minimum completion time is $3$ in this example. 
%----------------
%I hope I did not eliminate the sentences
%
%Please add it <= Ono sensei
%
%--------------------------

\medskip
\noindent
{\large\bf Applications and related work}: 
%\subsection*{Applications and Related work}
Reallocation scheduling is one of the most fundamental problems in various areas such as supply chain management, logistics, and transportation science.  Many models and variants of reallocation have been studied from both  theoretical and practical viewpoints. 
In fact, our problem setting is initiated by an industry-academia joint project of Advanced Mathematical Science for Mobility Society by Toyota Motor Corporation and Kyoto University~\cite{Toyota}.     
The reallocation models and their variants are categorized by the following aspects: (1) reallocation cost, (2) fungibility of  products, and (3) parallel/sequential execution.  
%(1) a cost of reallocating  products is a matter, or not, (2)  products are fungible or not, (3) reallocation can be done in a parallel way or only in a sequential way. (1) 
Our problem assumes that (1) a cost (i.e., transit time) of reallocating a product is given in advance, (2)  products are not fungible, 
and (3) reallocations are done in a parallel way, but many other settings are possible. 

For example, the dial-a-ride problem is regarded as the vehicle routing problem for reallocation~\cite{cordeau2007dial,ho2018survey}, which designs vehicle routes and schedules for customers  who request the pick-up and drop-off points. 
In the dial-a-ride problem, (1) the cost of reallocation depends on the routes, (2) customers are not fungible of course, (3) reallocation is done in a sequential way for one vehicle. 
The bike-sharing rebalancing problem is  to schedule trucks for re-distributing shared bikes with the objective of minimizing total cost~\cite{dell2014bike}. In the bike-sharing rebalancing problem, (1) the cost of reallocation also depends on the routes of trucks and (3) reallocation is done in a sequential way  for one truck again, but (2) shared bikes are fungible, i.e.,  the desired bike distribution is created without distinguishing between bikes.  
%In fact, the reallocation schedule models real-world problems discussed in a practically oriented project with Toyota Motor Corporation, which include reallocating shared cars in parking lots.    
%As an industry-academia joint project, Toyota Motor Corporation and Kyoto University recently launched a research unit of Advanced Mathematical Science for Mobility Society~\cite{Toyota}. In the project, several real-world problems other than above are realized to be modeled as reallocation scheduling, e.g., reallocating shared cars in parking slots. 
%Reallocating shared cars in parking slots is a similar problem, which is considered in an industry-academia joint project of Advanced Mathematical Science for Mobility Society by Toyota Motor Corporation and Kyoto University~\cite{Toyota}. In the problem, each car directly moves to another parking slot, whereas shared bikes are delivered by trucks along their routes. In the model, (2) cars are fungible in many cases, and thus (1) the reallocation cost depends only on the assignment of cars to the parking slots, and (3) reallocation is done in a parallel way.  

In these problems, the costs arise from rather transportation of vehicles for delivery than reallocation of  products.  
To investigate the nature of reallocation itself, it might be reasonable to assume that a cost (i.e., transit time) of reallocating a product is given in advance.   
%Not only that, the reallocation scheduling appears in various fields, such as memory allocation with limited buses and settlement fund circulation.  
Miwa and Ito \cite{miwa1996complexity,miwa1997linear,miwa2000np} focus on reallocation scheduling  under the setting: (1) a cost of reallocating  products is uniform, (2)  products are not fungible, 
and (3) reallocations are done in a sequential way, which is different from ours. 
%Miwa and Ito \cite{miwa1996complexity,miwa1997linear,miwa2000np} investigate the computational complexity of another type of reallocation scheduling, which computes how to move vacant spaces. 
Although they do not deal with non-uniform transition time, several intractability results as well as polynomial solvability ones  were obtained \cite{miwa1996complexity,miwa1997linear,miwa2000np}.  
A  problem similar to the model of Miwa and Ito was also considered in \cite{HAYAKAWA201986}, in the context of fund circulation. In \cite{hayakawa2018does,hayakawa2020liquidity}, Hayakawa pointed out the importance of controlling a payment ordering among banks in terms of the stability of economics, and introduced the problem to find a payment ordering that minimizes extra money to put in order to make payments without shortage, which can be viewed as a  reallocation scheduling problem. Here 
 the extra money corresponds to vacant spaces for the reallocation. 
From such a viewpoint, the computational complexity of the fund circulation was investigated in \cite{HAYAKAWA201986}.  


%Among many related studies, the last two above have similar features to our reallocation problem, though their concerns are different from ours in several aspects. For example, their models do not take into account transition time. Furthermore, their models  reallocate  products (or products, fund) in a step-by-step manner, whereas our model allows simultaneous reallocation. It yields a major difference in solution spaces.  As an example, consider  product $p_1$ in warehouse $W_1$ and  product $p_2$ in warehouse $W_2$ with an identical size $s$ and transition time $1$ need to be reallocated to warehouses $W_2$ and $W_3$, respectively. Warehouse $W_2$ has no vacancy, though Warehouse $W_3$ has vacant space with size $s$. In their models, $p_2$ should be first reallocated to the vacant space of $W_3$ and then $p_1$ is reallocated to the vacant space of $W_1$ in the next step. In our model, $p_1$ and $p_2$ are respectively reallocated to $W_2$ and $W_2$ in one step.  In the same instance above, we suppose that the vacant space with size $s$ of warehouse $W_3$ is replaced with  product $p_3$ of size $s$, which is designated to be $W_1$. If $W_1$ has no extra vacant space, the reallocation is impossible under their models, because no  product can be initially moved. On the other hand, it is feasible in our model by reallocating $p_1, p_2$ and $p_3$ to $W_2, W_3$ and $W_1$, respectively.  In \cite{miwa1996complexity,miwa1997linear,miwa2000np}, they show NP-hardness of general or restricted settings of the problem and present fast algorithms that solve some special cases. Hayakawa et al.  \cite{HAYAKAWA201986} investigate minimization and maximization of extra money (i.e., vacant spaces) for making the instance feasible, and give hardness results and polynomial-time solbability for general cases and several restricted cases.   

\medskip
\noindent
{\large\bf Our contribution}: 
%\subsection*{Our contribution} 
In this paper, we consider the reallocation scheduling in which  products are with fixed cost,  non-fungible, and reallocated  in parallel, which we simply call the {\em reallocation problem}. %where it is simply called the {\em reallocation problem}. 
We investigate the computational complexity of the reallocation problem under various scenarios. 
We first see the most basic scenario  where both the  product size and transition time are uniform. In this scenario, we present an $\mO(\ishii{mn} \log m)$-time algorithm to find a reallocation schedule with minimum completion time, where
$m$ and $n$ denote the number of  products and warehouses, respectively.
%$m$ denotes the number of  products. %More precisely, if $\tau(p)=1$ for every  product $p$, 
The algorithm utilizes a cycle decomposition for the so-called demand graph. 
When the  product size is only uniform, the problem turns out to be NP-hard, and we show that the algorithm for the basic scenario above provides a reallocation schedule 
whose completion time is at most twice the optimal, if one of the carry-out and carry-in capacities is sufficiently large in addition.
Here we note that the carry-in and carry-out capacity constraints are always %automatically 
satisfied if the carry-in and carry-out capacities are sufficiently large, respectively. 
For more general scenarios, even the feasibility is NP-complete for very restricted settings: (1) we have only two warehouses and (2) the transit time  and  the  product size satisfy
$\transit(p)=1$
and $\size(p) \in \{1,2\}$ for every  product $p$.
Due to the hardness of the feasibility, 
%we have no choice but to give up constructing %approximation algorithms for the reallocation problem. 
%polynomial-time algorithms with approximation guarantee for the problem as it is.    
no polynomial-time algorithm can construct a feasible schedule of the problem unless P$=$NP.  
Instead, 
we admit the relaxation of capacity constraints, which we call \emph{capacity augmentation}. 
Namely, we augment the original capacities with additional ones, and try to find a reallocation schedule such that it is feasible with the augmented instance and has small completion time. 
By utilizing the  bi-criteria algorithm schemes
%iterative approximation algorithms
 for the generalized assignment problem \cite{ST93} and the $2$-sided placement problem \cite{KMRT15},  
we can find in polynomial time  a reallocation schedule such that 
(i) the completion time is at most the minimum completion time for the original problem, (ii)  warehouses can be stored at most twice of the original capacities (i.e., warehouse capacity $c(w)$ is augmented with $c(w)$ for each warehouse $w$), 
and (iii) carry-out/in capacities are enlarged to the original ones plus the largest and second largest carried-out/in product sizes (i.e., the carry-out and carry-in capacities  for each warehouse $w$ are respectively augmented with 
$\sigma^+_1(w)+\sigma^+_2(w)$ and $\sigma^-_1(w)+\sigma^-_2(w)$, where $\sigma^+_i(w)$ and $\sigma^-_i(w)$ denote the $i$-th largest size of  products that are initially and finally stored in warehouse $w$, respectively). 
In the scenario when the carry-in (resp., carry-out) capacity is sufficiently large, condition (iii) is strengthened into the original carry-out (resp., carry-in) capacity plus the largest size of carry-out (resp., carry-in)  product size. 
We remark that if both carry-in and carry-out capacities are sufficiently large, the problem turns out to be trivial, where an optimal reallocation schedule can be obtained by sending all  products in time $0$. 
 Table \ref{tab:result0} summarizes the results above, i.e., for general warehouse capacity. 
%
\begin{table}[thbp]
    \caption{The summary of results for general warehouse capacity.  } 
    \scriptsize
    \label{tab:result0}
    \begin{center}
    \begin{tabular}{|c|c|c|c||c|c|}\hline 
     product & transition & \multicolumn{2}{c||}{capacity} & \multirow{2}{*}{complexity $\&$} & \multirow{3}{*}{capacity augmentation$^\dagger$}\\ \cline{3 - 4}   
     size & time  & carry-out & carry-in& \multirow{2}{*}{approximability$^*$}&\\ 
     ($size(p)$) & ($\tau(p)$) & ($d^+$) & ($d^-$)  & &\\  \hline \hline 
    \multirow{2}{*}{uniform} & \multirow{2}{*}{uniform}  & \multirow{2}{*}{general} & \multirow{2}{*}{general} & $\mO(\ishii{mn \log m})$ & \multirow{2}{*}{---------}\\ 
    &&&&[Th. \ref{poly:th}]&\\\hline
    \multirow{2}{*}{uniform} & \multirow{2}{*}{general}  & general & $+\infty$ &  2-apx &\multirow{2}{*}{---------}\\  
      &  & $(+\infty$ & general) & [\ishii{Th. \ref{2apx:th}}]&\\ \hline
   \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} &  NPH &\multirow{2}{*}{---------}\\ 
   &&&&[\ishii{Th \ref{flowshop:th}}]&\\ \hline
      \multirow{2}{*}{general} & \multirow{2}{*}{general}    & \multirow{2}{*}{$+\infty$} & \multirow{2}{*}{$+\infty$} & $\mO(m+n)$& \multirow{2}{*}{---------} \\ 
     &&&&[\ishii{Th. \ref{trivial:th}}]&\\\hline
   %
   &&&&&$\hat{c}=2c$\\
   \multirow{2}{*}{general} & \multirow{2}{*}{uniform} & general &$+\infty$ & NPC &$\hat{d}^+=d^++\sigma^+_1$\\  
      &  & $(+\infty$ & general) & [Th. \ref{hard1:th}]&($\hat{d}^-=d^-+\sigma^-_1$)\\ 
      &&&&&[Th.~\ref{bicriteria:th} (ii)]\\ \hline
    %
    &&&&&$\hat{c}=2c$ \\
    \multirow{2}{*}{general} & \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & NPC &$\hat{d}^+=d^++\sigma^+_1+\sigma^+_2$\\ 
      &  & & &[Th. \ref{hard1:th}]&$\hat{d}^-=d^-+\sigma^-_1+\sigma^-_2$\\ 
      &&&&&[Th.~\ref{bicriteria:th} (i)]\\
      \hline
    %  
    &&&&&$\hat{c}=2c$\\
   \multirow{2}{*}{general} & \multirow{2}{*}{general}  & general & $+\infty$ & 
   NPC &$\hat{d}^+=d^++\sigma^+_1$\\  
      &  & ($+\infty$ & general) & [Th. \ref{hard1:th}]&($\hat{d}^-=d^-+\sigma^-_1$)\\ 
      &&&&&[Th.~\ref{bicriteria:th} (ii)]\\\hline
%      
     & & &   & &$\hat{c}=2c$ \\ 
 \multirow{2}{*}{general}& \multirow{2}{*}{general}&\multirow{2}{*}{general}&\multirow{2}{*}{general}&NPC&$\hat{d}^+=d^++\sigma^+_1+\sigma^+_2$ \\
    &&&&[Th. \ref{hard1:th}]&$\hat{d}^-=d^-+\sigma^-_1+\sigma^-_2$\\
    &&&&&[Th.~\ref{bicriteria:th} (i)]\\ \hline  
    \end{tabular}
    \end{center}
    $^*$: ``NPC'' stands for  NP-completeness of the feasibility of the reallocation problem and ``NPH'' stands for NP-hardness for the reallocation problem.\\
    $^\dagger$: $\hat{c}$, $\hat{d}^+$, and $\hat{d}^-$ respectively denote augmented warehouse, carry-out, and carry-in capacities.
\end{table}
%
\nop{
\begin{table}[htbp]
    \caption{The summary of results: Complexity and Approximability. } 
    \scriptsize
    \label{tab:result1}
    \begin{center}
    \begin{tabular}{|l|l|c|c|c||c|c|}\hline 
     product & transition & \multicolumn{3}{c||}{capacity} & \multirow{2}{*}{complexity $\&$} & \multirow{2}{*}{capacity}\\ \cline{3 - 5}   
     size & time & warehouse & carry-out & carry-in& \multirow{2}{*}{approximability}&\multirow{2}{*}{augmentation}\\ 
     ($size(p)$) & ($\tau(p)$) & ($c(w)$) & ($d^+$) & ($d^-$)  & &\\  \hline \hline 
    \multirow{2}{*}{uniform} & \multirow{2}{*}{uniform}  & \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & $O(m \log m)$ & \multirow{2}{*}{---------}\\ 
    &&&&&[Th. \ref{poly:th}]&\\\hline
    \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & general & $+\infty$ &  2-apx &\multirow{2}{*}{---------}\\  
    &  &  & $(+\infty$ & general) & [Th. \ref{???}]&\\ \hline
   \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} &  NPH$^\dagger$ &\multirow{2}{*}{---------}\\ 
   &&&&&[Th \ref{}]&\\ \hline
    \multirow{2}{*}{general} & \multirow{2}{*}{general}  & \multirow{2}{*}{general}   & \multirow{2}{*}{$+\infty$} & \multirow{2}{*}{$+\infty$} & $O(m+n)$& \multirow{2}{*}{---------} \\ 
     &&&&&[Th. \ref{irukana?? dousuru}]&\\\hline
   \multirow{2}{*}{general} & \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & general & $+\infty$ & NPC$^*$ &\\  
    &  &  & $(+\infty$ & general) & [Th. \ref{hardness1:subsec}]&\\ \hline
    \multirow{2}{*}{general} & \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & NPC$^*$ &\\ 
    &  &  & & &[Th. \ref{hardness1:subsec}]&\\ \hline
   \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & general & $+\infty$ & 
   NPC$^*$ &\\  
    &  &  & $(+\infty$ & general) & [Th. \ref{hardness1:subsec}]&\\ \hline
    \multirow{3}{*}{general} & \multirow{3}{*}{general} & \multirow{3}{*}{general} & \multirow{3}{*}{general} & \multirow{3}{*}{general}  & \multirow{2}{*}{NPC$^*$}&$\hat{c}(w)=2c(w)$ \\ 
    &&&&&\multirow{2}{*}{[Th. \ref{hardness1:subsec}]}&$\hat{d}^+(w)=d(w)+\sigma(w)+\sigma(w)$\\
    &&&&&&\\ \hline  
    \end{tabular}
    \end{center}
    $^*$: ``NPC'' stands for  NP-completeness of the feasibility of the reallocation problem.\\
    $^\dagger$: ``NPH'' stands for NP-hardness for the reallocation problem. 
\end{table}
}
%
\begin{table}[hbtp]
    \caption{The summary of results for 
    %uniform
    \ishii{sufficiently large}
    warehouse capacity.  } 
    \small
    \label{tab:result1}
    \begin{center}
    \begin{tabular}{|c|c|c|c||c|}\hline 
     product &  transition & \multicolumn{2}{c||}{capacity} & \multirow{3}{*}{complexity $\&$ approximability$^*$} \\ \cline{3 - 4}   
     size & time  & carry-out & carry-in& \\ 
     ($size(p)$) & ($\tau(p)$)  & ($d^+$) & ($d^-$)  & \\  \hline \hline 
   \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & general & $+\infty$ & \multirow{2}{*}{\ishii{$\mO(n+m\log{m})$}  [\ishii{Th. \ref{apx:th}(i)}]}\\  
      &  & $(+\infty$ & general) & 
   \\ \hline
   \multirow{2}{*}{uniform} & \multirow{2}{*}{general}  & \multirow{2}{*}{general} & \multirow{2}{*}{general}  & NPH  [\ishii{Th \ref{flowshop:th}}] \\ 
   &&&&\ishii{4-apx} [Th. \ref{apx:th}\ishii{(iv)}] \\ \hline
   \multirow{2}{*}{general} & \multirow{2}{*}{uniform}  & general & $+\infty$ & NPH [Th. \ref{hard2:th}]\\  
      &  & $(+\infty$ & general) &  3/2-apx  (tight) [Ths. \ref{apx:th}\ishii{(ii)},\ref{binpack1:th}]\\ \hline
    \multirow{2}{*}{general} & \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{general}  & NPH [Th. \ref{hard2:th}]\\
    &&&& 6-apx [Th. \ref{apx:th}\ishii{(v)}]\\ \hline
 \multirow{2}{*}{general} & \multirow{2}{*}{general} & general & $+\infty$ & NPH [Th. \ref{hard2:th}] \\  
      &  & $(+\infty$ & general) &  7/4-apx [Th. \ref{apx:th}\ishii{(iii)}] \\ \hline
    \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general}  & NPH [Th. \ref{hard2:th}]\\
    &&&& 6-apx [Th. \ref{apx:th}\ishii{(v)}]\\ \hline 
    \end{tabular}
    \end{center}
    $^*$: ``NPH'' stands for NP-hardness for the reallocation problem. 
\end{table}
%We also show that our problem is NP-hard, even if the  product size is uniform, 
%which together with the positive result and (2) mentioned above  provides a sharp boundary for the complexity  of our problem. 
%Namely, it is polynomially solvable if the transit time and  product size are both uniform, 
%and it NP-hard if at least one of them is not uniform.  



We finally consider the scenario when all warehouses have sufficiently large capacities, where the summary of our results can be found in Table \ref{tab:result1}.  
In this setting, we propose a $6$-approximation algorithm for our problem that transforms a {\em relaxed} schedule above %the above  bi-criteria-type algorithm
into a feasible schedule such that the completion time is at most 6 times of the minimum completion time. 
In the setting when  at least one of  carry-in and  carry-out capacities is sufficiently large in addition, we present a  $7/4$-approximation algorithm that employs as a subroutine the first-fit-decreasing algorithm for the bin packing problem. 
If we further assume that the transition time is uniform, the approximation ratio is improved to $3/2$, which is best possible in the setting. 
This follows from the fact that the problem in this setting  is essentially equivalent to the bin packing problem. 
We also show that the reallocation problem can be solved in polynomial time, if the  product size is uniform and at least one of the carry-in and carry-out capacities are sufficiently large in addition. 

%Our results are summarized in Tables \ref{tab:result1} and %\ref{tab:result2}. 
%Table \ref{tab:result1} summarizes the results about the time complexity and approximability. 



%Table \ref{tab:result2} summarizes the results about capacity augmentation. 

\nop{%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
    \caption{The summary of results: Complexity and Approximability. } 
    \small
    \label{tab:result1}
    \begin{center}
    \begin{tabular}{|l|l|c|c|c||l|}\hline 
     product &  transition & \multicolumn{3}{c||}{capacity} & \multirow{3}{*}{complexity and approximability$^*$} \\ \cline{3 - 5}   
     size & time & warehouse & carry-out & carry-in& \\ 
     ($size(p)$) & ($\tau(p)$) & ($c(w)$) & ($d^+$) & ($d^-$)  & \\  \hline \hline 
    uniform & uniform  & general & general & general & $O(m \log m)$ [Th. \ref{poly:th}] \\ \hline
     general &  general  & general & $+\infty$ & $+\infty$ & $O(m+n)$  \\ \hline
    \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & general & $+\infty$ &  \ishii{hardness??, 2-apx [algorithm of Th. \ref{poly:th}]}\\  
    &  &  & $(+\infty$ & general) & \\ \hline
   uniform & general & general & general & general  &  \ishii{S-NPH [flowshop]}\\ \hline
   \multirow{2}{*}{general} & \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & general & $+\infty$ & \ishii{S-NPc [Th. \ref{hardness1:subsec}]}\\  
    &  &  & $(+\infty$ & general) & \\ \hline
    general & uniform & general & general & general  & \ishii{S-NPc [Th. \ref{hardness1:subsec}]}\\ \hline
   \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & general & $+\infty$ & \ishii{S-NPc [Th. \ref{hardness1:subsec}]}\\  
    &  &  & $(+\infty$ & general) & \\ \hline
    general & general & general & general & general  & \ishii{S-NPc [Th. \ref{hardness1:subsec}]}\\ \hline  
  \multirow{2}{*}{uniform} & \multirow{2}{*}{general} & \multirow{2}{*}{$+\infty$} & general & $+\infty$ & \ishii{P?? (sending   products in nonincreasing order of $\transit$)}\\  
    &  &  & $(+\infty$ & general) & 
    \ishii{(7/4-apx [Th. \ref{apx:th}(ii)])}\\ \hline
   uniform & general & $+\infty$ & general & general  & \ishii{S-NPH [flowshop], 6-apx [Th. \ref{apx:th}(iii)]}\\ \hline
   \multirow{2}{*}{general} & \multirow{2}{*}{uniform} & \multirow{2}{*}{$+\infty$} & general & $+\infty$ & \ishii{S-NPH [Th. \ref{hard2:th}], (3/2-$\varepsilon$)-inapx [Th. \ref{binpack1:th}]}\\  
    &  &  & $(+\infty$ & general) &  \ishii{3/2-apx [Th. \ref{apx:th}(i)]}\\ \hline
    general & uniform & $+\infty$ & general & general  & \ishii{S-NPH [Th. \ref{hard2:th}], 6-apx [Th. \ref{apx:th}(iii)]}\\ \hline
 \multirow{2}{*}{general} & \multirow{2}{*}{general} & \multirow{2}{*}{$+\infty$} & general & $+\infty$ & \ishii{S-NPH [Th. \ref{hard2:th}],\ (3/2-$\varepsilon$)-inapx [Th. \ref{binpack1:th}]}\\  
    &  &  & $(+\infty$ & general) &  \ishii{7/4-apx [Th. \ref{apx:th}(ii)]} \\ \hline
    general & general & $+\infty$ & general & general  & \ishii{S-NPH [Th. \ref{hard2:th}], 6-apx [Th. \ref{apx:th}(iii)]}\\ \hline 
    \end{tabular}
    \end{center}
    $^*$: ``S-NPc'' stands for strong NP-completeness of the feasibility, and ``S-NPH'' stands for strong NP-hardness for optimization. 
\end{table}
}
\nop{

\begin{table}[htbp]
    \caption{The summary of results: Complexity and Approximability. } 
    \small
    \label{tab:result1}
    \begin{center}
    \begin{tabular}{|l|l|c|c|c||l|}\hline 
     product &  transition & \multicolumn{3}{c||}{capacity} & \multirow{3}{*}{complexity and approximability$^*$} \\ \cline{3 - 5}   
     size & time & warehouse & carry-out & carry-in& \\ 
     ($size(p)$) & ($\tau(p)$) & ($c(w)$) & ($d^+$) & ($d^-$)  & \\  \hline \hline 
    uniform & \multirow{6}{*}{uniform}  & \multirow{4}{*}{general} & \multirow{1}{*}{general} & \multirow{1}{*}{general} & $O(m \log m)$ [Theorem \ref{poly:th}] \\ \cline{1-1}\cline{4-6}
    $\{1,2\}$ &  &  &  &  & S-NPC [Theorem \ref{size12:th}]\\ \cline{1-1} \cline{6-6}  
        \multirow{6}{*}{general}  &  &  & &  & S-NPC for $|W|=2$ [Theorem \ref{hard1:th}]\\  
        &  & \multirow{5}{*}{$\infty$} & general & $\infty$ & $(3/2-\varepsilon)$-inapprox. [Theorem \ref{binpack1:th}]\\  \cline{3-3} \cline{6-6} 
            &  &  &  /$\infty$ &  /general  & S-NPH for $|W|=2$ [Theorem \ref{hard2:th}]\\ 
            &  &  &  &  & $3/2$-approx. [Theorem \ref{apx:th} (i)] \\ \cline{2-2} \cline{6-6} 
            & \multirow{2}{*}{general} &  &  &  & $7/4$-approx. [Theorem \ref{apx:th} (ii)]\\ \cline{4-6}  
            &   &  & general  & general & $6$-approx. [Theorem \ref{apx:th} (iii)] \\
        \hline
    \end{tabular}
    \end{center}
    $^*$: ``S-NPc'' stands for strong NP-completeness of the feasibility, and ``S-NPH'' stands for strong NP-hardness for optimization. 
\end{table}

\begin{table}[htbp]
    \caption{The summary of results: capacity augmentation.}\label{tab:result2}
    \small
    \begin{center}
    \begin{tabular}{|l|l|c|c|c||l|}\hline 
     product &  transition & \multicolumn{3}{c||}{capacity} & \multirow{3}{*}{capacity augmentation$^{\dagger}$ } \\ \cline{3 - 5}   
     size & time & warehouse & carry-out & carry-in& \\ 
     ($size(p)$) & $ (\tau(p)$) & ($c(w)$) & ($d^+$) & ($d^-$)  & \\  \hline \hline 
    \multirow{4}{*}{general} & \multirow{4}{*}{general} & \multirow{4}{*}{$\infty$} & \multirow{2}{*}{general} & \multirow{2}{*}{general} & $d^+$ \verb|+=| $\sigma^+_1+\sigma^+_2$, $d^-$ \verb|+=| $\sigma^-_1+\sigma^-_2$, \\  
         &  &  &  &  & $c(w)$ \verb|+=| $c(w)$ [Theorem \ref{bicriteria:th} (i)]\\  \cline{4-6}
            &   &  & $\infty$ & general & $d^-$ \verb|+=| $\sigma^-_1$ [Theorem \ref{bicriteria:th} (ii)] \\
        \cline{4-6}
            &   &  & general & $\infty$ & $d^+$ \verb|+=| $\sigma^+_1$ [Theorem \ref{bicriteria:th} (ii)] \\
        \hline
    \end{tabular}
    \end{center}
    $^{\dagger}$: ``\emph{parameter} \verb|+=|\emph{value}'' represents that there is an algorithm that can find a schedule with $ALG\le OPT$ under the setting that \emph{parameter} is augmented with \emph{value}, where $ALG$ is the completion time found by the algorithm and $OPT$ is the minimum completion time of the original instance.
\end{table}
\bigskip 
}
The rest of the paper is organized as follows. In Section \ref{preliminaries:sec}, 
%we formally define the problem and give a basic observation about the capacity constraints. 
we give formal definitions and basic observations. 
Section \ref{size2:sec}  presents a polynomial-time algorithm for the setting where both  size and transition time of products are uniform. 
Section \ref{bicriteria:sec} considers the most general setting; we introduce a notion of capacity augmentation, and present a polynomial-time algorithm 
%for the reallocation schedule of minimum completion time 
under augmented capacities. 
In Section \ref{nocap:sec}, we consider the setting where the capacities of warehouses are sufficiently large, and present constant-factor approximation algorithms for the setting. Section \ref{hardness:sec} summarizes hardness results in various settings. Due to the space limitation, we omit most of the detailed proofs, which can be seen in Appendix.   
